Carryless Arithmetic Mod 10

We investigate what arithmetic would look like if carry digits into other digit position were ignored, so that 9 + 4 = 3, 5 + 5 = 0, 9 X 4 = 6, 5 X 4 = 0, and so on. For example, the primes are now 21, 23, 25, 27, 29, 41, 43, 45, 47, ... .

==> cross.latex <==
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1062,1062)(1270,-1492)
{\color[rgb]{0,0,0}\put(1483,-431){\line( 1,-1){848}}
\multiput(2331,-1279)(-6.05714,-6.05714){36}{\makebox(0.0000,0.0000){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\put(2119,-1491){\line(-1, 1){848}}
\multiput(1271,-643)(6.05714,6.05714){36}{\makebox(0.0000,0.0000){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
}%
{\color[rgb]{0,0,0}\multiput(2119,-431)(6.05714,-6.05714){36}{\makebox(0.0000,0.0000){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\put(2331,-643){\line(-1,-1){848}}
\multiput(1483,-1491)(-6.05714,6.05714){36}{\makebox(0.0000,0.0000){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\put(1271,-1279){\line( 1, 1){848}}
}%
\end{picture}%


==> plus.latex <==
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1202,1202)(1200,-1562)
{\color[rgb]{0,0,0}\put(1201,-1111){\framebox(1200,300){}}
}%
{\color[rgb]{0,0,0}\put(1651,-1561){\framebox(300,1200){}}
}%
\end{picture}%

